Covert Communications through Imperfect Cancellation

We propose a method for covert communications using an IEEE 802.11 OFDM/QAM packet as a carrier. We show how to hide the covert message so that the transmitted signal does not violate the spectral mask specified by the standard, and we determine its impact on the OFDM packet error rate. We show conditions under which the hidden signal is not usable and those under which it can be retrieved with a usable bit error rate (BER). The hidden signal is extracted by cancellation of the OFDM signal in the covert receiver. We explore the effects of the hidden signal on OFDM parameter estimation and the covert signal BER. We conclude with an experiment using Over-The-Air recordings of 802.11 packets, inject the hidden

==> mathalpha/README <==
______________________________________
The MATHALPHA (*AKA MATHALFA) package

As of version 1.12, the name of the package mathalfa was changed to mathalpha. (When I made the first version over 10 years ago, 8.3 filenames were still preferred iny a few older systems, leasing to what might appear as an unfortunate error in English spelling.) This should make no difference in its usage---though the name is changed, it works the same under both names. On CTAN, though the package will be set up as mathalpha, an alias will find it under the name mathalfa. The documentation name has been changed to mathalpha-doc.{tex,pdf} so some changes in texdoc data and the like will be necessary.

This package provides a standard means of setting math alphabets 
associated with the macros \mathcal, \mathbb, \mathfrak and \mathscr
and, where available, their bold counterparts \mathbcal, \mathbbb, 
\mathbfrak and \mathbscr. 
It mostly bypasses the usual fd and sty files used to load these 
alphabets in order to allow each to be scaled independently and 
without silently quantizing the sizes.

Version 1.13 changes the behavior under the option scr, first letting \mathscr to \relax, in case it was previously defined. This corrects a misbehavior under newtxmath 1.6 and newpxmath 1.4. (*)Thanks Evan Couch.)

Version 1.12 Name of package changed from mathalfa to mathalpha.

Version 1.11 adds the option scr=kp to point to kpfonts script alphabet. It also introduces a new name for the package, though you may call by either name, whichever is less offensive to you.

Version 1.10 adds the option bb=dsserif to point to the new DSSerif font.

Version 1.09 adds two more calligraphic/script alphabets, both upright---txupr is based on the math calligraphic font from the TX fonts, and boondoxupr is derived from the stix math script fonts, version 1.1.

Version 1.08 adds two more alphabets---bb=libus sets blackboard bold to the double-struck alphabet from LibertinusT1Math, and cal=stix sets the calligraphic alphabet to the one in stix-mathcal.pfb.

Copyright 2012--2019 Michael Sharpe
msharpe at ucsd dot edu

License: 
  This work may be distributed and/or modified under the
  conditions of the LaTeX Project Public License, either
  version 1.3c of this license or (at your option) any 
  later version: <http://www.latex-project.org/lppl.txt>
____________________

